Agentic AI: The Era of Semantic Decoding

Recent work demonstrated great promise in the idea of orchestrating collaborations between LLMs, human input, and various tools to address the inherent limitations of LLMs. We propose a novel perspective called semantic decoding, which frames these collaborative processes as optimization procedures in semantic space. Specifically, we conceptualize LLMs as semantic processors that manipulate meaningful pieces of information that we call semantic tokens (known thoughts). LLMs are among a large pool of other semantic processors, including humans and tools, such as search engines or code executors. Collectively, semantic processors engage in dynamic exchanges of semantic tokens to progressively construct high-utility outputs. We refer to these orchestrated interactions among semantic processors, optimizing and searching in semantic space, as semantic decoding algorithms. This concept draws a direct parallel to the well-studied problem of syntactic decoding, which involves crafting algorithms to best exploit auto-regressive language models for extracting high-utility sequences of syntactic tokens. By focusing on the semantic level and disregarding syntactic details, we gain a fresh perspective on the engineering of AI systems, enabling us to imagine systems with much greater complexity and capabilities. In this position paper, we formalize the transition from syntactic to semantic tokens as well as the analogy between syntactic and semantic decoding. Subsequently, we explore the possibilities of optimizing within the space of semantic tokens via semantic decoding algorithms. We conclude with a list of research opportunities and questions arising from this fresh perspective. The semantic decoding perspective offers a powerful abstraction for search and optimization directly in the space of meaningful concepts, with semantic tokens as the fundamental units of a new type of computation.

==> 08_ethics.tex <==
% Important ethical considerations arise from the development and deployment of AI technologies. The collaborative nature of semantic decoding algorithms, involving interactions between humans, large language models (LLMs), and various tools, presents both opportunities and risks. Understanding and mitigating these risks is essential to ensure the responsible development and deployment of semantic decoding algorithms.

% Collaborative AI systems typically leverage pre-trained language models as their main semantic processors. Consequently, semantic decoding algorithms inherit risks and ethical concerns stemming from language models. In \Secref{05_applications}, we discuss how collaborative systems can potentially utilize dedicated semantic processors to address and mitigate some of the issues associated with LLMs, such as unethical, biased, or unfair outcomes. These solutions require conscious efforts from developers to investigate the presence of such problems and craft dedicated semantic processors to mitigate them. 

% Issues of transparency, accountability, and data privacy in the development and deployment of language models directly extend to collaborative systems relying on them, especially when these models are proprietary commercial systems hidden behind APIs.

% Without adequate safeguards, sensitive information shared during collaboration could be compromised, leading to privacy breaches and violations of data protection regulations. Protecting privacy and data rights necessitates robust data anonymization techniques, informed consent for data collection and usage, and adherence to relevant legal and regulatory frameworks. This highlights the need for research to ensure private participation in semantic decoding computations.

% Collaborative AI technologies, like other impactful technologies, have the potential to profoundly transform society, impacting employment, inequality, and misinformation. As researchers and developers, we have a responsibility to anticipate and mitigate potential negative societal impacts at every stage of the research and development pipelines, ensuring that collaborative AI technologies serve broader interests.

% The inclusion of humans in collaborative AI systems can have significant psychological impacts, influencing individuals' perceptions of autonomy, competence, and trust in technology. Involving humans in AI decision-making processes may lead to feelings of empowerment and control, as users become active participants in shaping outcomes. However, it can also raise concerns about accountability, especially if users perceive AI systems as opaque or difficult to understand. Addressing these psychological impacts requires careful consideration of inclusivity, particularly regarding language barriers and accessibility.

% In conclusion, addressing ethical considerations requires prioritizing transparency, fairness, privacy, societal impact, human empowerment, accountability, and inclusivity. The framework of semantic decoding is well-suited to tackle these issues and incorporate proper, human-interpretable safeguards.
